Generating Multi-Aspect Queries for Conversational Search

Conversational information seeking (CIS) systems aim to model the user's information need within the conversational context and retrieve the relevant information. One major approach to modeling the conversational context aims to rewrite the user utterance in the conversation to represent the information need independently. Recent work has shown the benefit of expanding the rewritten utterance with relevant terms. In this work, we hypothesize that breaking down the information of an utterance into multi-aspect rewritten queries can lead to more effective retrieval performance. This is more evident in more complex utterances that require gathering evidence from various information sources, where a single query rewrite or query representation cannot capture the complexity of the utterance. To test this hypothesis, we conduct extensive experiments on five widely used CIS datasets where we leverage LLMs to generate multi-aspect queries to represent the information need for each utterance in multiple query rewrites. We show that, for most of the utterances, the same retrieval model would perform better with more than one rewritten query by 85% in terms of nDCG@3. We further propose a multi-aspect query generation and retrieval framework, called MQ4CS. Our extensive experiments show that MQ4CS outperforms the state-of-the-art query rewriting methods. We make our code and our new dataset of generated multi-aspect queries publicly available.

==> tables/ablation-example.tex <==



\begin{table}[t]
\small
\centering
\caption{Example of queries and answers generated in Oracle version of \gptF-\AQD approach from \ikat 23 dataset.}
\vspace{-2mm}
\label{tab:ablation-example}
\adjustbox{max width=0.5\textwidth}{
 \begin{tabular}{p{7cm}}
\toprule
\textbf{Utterance:} How about their screen resolution? Are any of them better than what I  have?\\ 
\midrule
\textbf{Human resolved:} How about their screen resolution? Are any of the \textcolor{color1}{Samsung Galaxy S22}, \textcolor{color2}{Xiaomi 12 and 12 Pro}, and \textcolor{color3}{OPPO Find X5 Pro} better than Samsung Galaxy Note 10 in terms of screen resolution?\\ 
\midrule
\textbf{$r^{\prime}$}: To check if any of the phone's screen resolution is better than your current one, I would need to know what phone and model you have. However, \textcolor{color1}{The Samsung Galaxy S22 has a screen resolution of 2340 x 1080 pixels}, \textcolor{color2}{Xiaomi 12 and 12 Pro have a resolution of 3200 x 1440 pixels}, and \textcolor{color3}{OPPO Find X5 Pro boasts a resolution of 3216 x 1440 pixels}.\\ 
\midrule
\textbf{$q_1$}. What is the screen resolution of \textcolor{color1}{Samsung Galaxy S22}?\newline
\textbf{$q_2$}. What is the screen resolution of \textcolor{color2}{Xiaomi 12 and 12 Pro}?\newline
\textbf{$q_3$}. What is the screen resolution of \textcolor{color3}{OPPO Find X5 Pro}?\newline
\textbf{$q_4$}.Are the screen resolutions of \textcolor{color1}{Samsung Galaxy  S22}, \textcolor{color2}{Xiaomi 12 and 12 Pro}, \textcolor{color3}{OPPO Find X5 Pro} high-definition?\newline
\textbf{$q_5$}. How does the screen resolution of \textcolor{color1}{Samsung Galaxy S22}, \textcolor{color2}{Xiaomi 12 and 12 Pro}, \textcolor{color3}{OPPO Find X5 Pro} compare to each other? \\
\bottomrule
\end{tabular}

}

\end{table}







 

==> tables/ablation-query-count.tex <==



\begin{table}[t]
\centering
\caption{Average of the optimal value of $\phi$ parameter for each user utterance in our datasets.}
\vspace{-2mm}
\label{tab:ablation-one-retrieval}
\adjustbox{max width=0.5\textwidth}{
 \begin{tabular}{lllll}
\toprule
Model & Dataset &    nDCG@3  &    R@10  &  R@100  \\
\toprule
\multirow{3}{*}{\AQD}  & \ikat 23  &  \textbf{2.965}  &   \textbf{2.936}  &  2.968   \\
\cmidrule{2-5}
  & \cast 22  &  2.774  &  2.756  &  2.893  \\
\cmidrule{2-5}  
  & \cast 20  &  2.832  &  2.839  &  \textbf{3.146}   \\
\midrule
\multirow{3}{*}{\QD} & \ikat 23  &  \textbf{3.013}  &  \textbf{2.956}  &  \textbf{2.926}   \\
\cmidrule{2-5}
& \cast 22   &  2.852  &  2.768  &  2.895  \\
\cmidrule{2-5}
& \cast 20   &  2.815  &  2.753  &  2.888    \\

\bottomrule
\end{tabular}

}

\end{table}







 

==> tables/ablation-retrieval-one.tex <==
\begin{table}[t]
\centering
\caption{Retrieval performance of \llama model in \AQD method using answer generated by \gptF compared to using answer generated by \llama. The results are comparable to \llama-\AQD from the main results table.}
\vspace{-2mm}
\label{tab:ablation-one-retrieval}
\adjustbox{max width=0.5\textwidth}{
 \begin{tabular}{lllllll}
\toprule
\textbf{Dataset} &  \textbf{nDCG@3} & \textbf{nDCG} & \textbf{R@10} & \textbf{R@100} & \textbf{MRR} \\
\toprule
\ikat 23   & 19.9  & 20.6  & 5.4  & 16.4  & 42.5 \\
\cast 22   & 16.2  & 29.9  & 4.5  & 20.2  & 39.1  \\
\cast 20   & 15.5  & 37.1  & 8.5  & 37.3  & 39.0  \\

\bottomrule
\end{tabular}

}

\end{table}





==> tables/ranking-main-pool-ikat.tex <==
\begin{table}[t]
% \fontsize{16pt}{16pt}\selectfont

\centering
\caption{Passage retrieval results on TREC \ikat 2023 dataset. The best results that are significantly (t-test $p\_value \leq 0.05$) better are indicated by \textbf{$^{\ast}$}. The best results are shown in \textbf{bold} and the second best results are shown with \underline{underline}. In these experiments, we use the $\phi=5$.}
\vspace{-2mm}
\label{tab:retrieval-results-main-pool-ikat}
\adjustbox{max width=0.5\textwidth}{
 \begin{tabular}{lllll}
\toprule
\textbf{Method} & \textbf{nDCG@3} & \textbf{R@10} & \textbf{R@100} & \textbf{MRR} \\
\toprule

\GPTFQR  & 21.9  & 9.3   & 22.1  & 34.6       \\
T5QR    & 14.1  & 5.8   & 13.8  & 23.9     \\
\ConvGQR   & 14.7  & 4.4   & 13.9  & 21.9       \\
\llamaQR  & 9.6   & 3.8   & 14.2  & 16.0   \\
\midrule
HumanQR  & 30.7  & 14.3  & 35.8  & 43.3          \\
\midrule
\gptF-\AD  & 15.0  & 7.0   & 22.2  & 24.6  \\
\gptF-\AQD  & 23.0  & 9.2   & 26.7  & 38.6   \\  
\gptF-\AQDAnswer & 18.1  & 6.5   & 25.2  & 30.6  \\
 \gptF-\QD   & 22.6  & 8.5   & 29.8  & 41.9   \\

\midrule
\llama-\AD  & 13.0  & 5.4   & 18.4  & 21.8     \\
\llama-\AQD  & 12.8  & 4.7   & 17.4  & 20.7     \\
\llama-\AQDAnswer  & 11.8  & 4.4   & 17.6  & 18.8     \\
 \llama-\QD   & 6.2   & 1.9   & 14.8  & 12.1     \\
\midrule
 \multicolumn{5}{c}{\textbf{Oracle}} \\
\midrule
 \gptF-\AQD      &  0.406  &  0.166  &  0.376  &  0.575 \\
\gptF-\AQDAnswer & 0.342  &  0.134  &  0.374  &  0.508   \\
\gptF-\QD       & 0.377  &  0.145  &  0.36  &  0.564 \\

\bottomrule


\end{tabular}

}

\end{table}
 




==> tables/ranking-with-SPLADE.tex <==
% \begin{table*}[t]
% \centering
% \caption{Passage retrieval results on TREC \cast 2020 and 2022 datasets. The best results that are significantly (t-test $p\_value \leq 0.05$) better are indicated by \textbf{$^{\ast}$} (Our comparison doesn't include the LLM4CS model). The best results are shown in \textbf{bold} and the second best results are shown with \underline{underline}. The best result outperforming all models is indicated by \textbf{$^{\ast}$}. The results for the LLM4CS model are reported from the original paper. In these experiments, we use the $\phi=5$.}
% \vspace{-2mm}
% \label{tab:retrieval-results-main-pool-cast}
% \adjustbox{max width=1\textwidth}{
%  \begin{tabular}{llllllllllll}
% \toprule
% \multirow{16}{*}{\rotatebox{90}{\textbf{Sparse (BM25)}}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{\cast 2020}} & & \multicolumn{4}{c}{\textbf{\cast 2022}}\\ \cmidrule{3-6} \cmidrule{8-11}

% &                     & \textbf{nDCG@3} &  \textbf{R@10} & \textbf{R@100} & \textbf{MRR} & & \textbf{nDCG@3} & \textbf{R@10} & \textbf{R@100} & \textbf{MRR}  \\
% \cmidrule(lr){1-11} % similar way to create ctoprule(2-11)
% &GPT4QR   & 46.8  & 24.4  & 55.2  & 61.5   && 34.8  & 9.6   & 30.1  & 52.2   \\
% &T5QR     & 38.7  & 19.6  & 45.6  & 53.1   && 30.2  & 8.1   & 23.9  & 45.5   \\
% &ConvGQR  & 35.7  & 19.1  & 47.7  & 49.4   && 25.0  & 6.6   & 22.1  & 41.0   \\
% &LLaMAQR  & 33.3  & 16.9  & 44.0  & 46.0   && 22.1  & 6.5   & 21.8  & 39.3   \\
% &LLM4CS   & 45.5  & -     & 48.9  & 61.5   &&  -    &   -   &  -    &  -   \\
% \cmidrule{2-11}
% &HumanQR    & 50.5  & 27.4  & 61.8  & 66.8   && 41.3  & 13.7  & 37.6  & 60.4   \\
% \cmidrule{2-11}
% &\gptF-\AD   & 45.2  & 23.6  & 54.6  & 62.3   && 31.3  & 10.2  & 32.5  & 49.9   \\
% &\gptF-\AQD  & 44.8  & 25.8  & 63.8  & 66.5   && 33.2  & 8.7   & 33.8  & 57.9   \\
% &\gptF-\AQDAnswer & 45.0  & 24.7  & 57.6  & 62.9   && 32.5  & 10.2  & 35.0  & 51.6   \\
% &\gptF-\QD   & 44.8  & 25.5  & 64.8  & 64.3   && 35.0  & 10.9  & 36.9  & 58.5   \\
% \cmidrule{2-11}
% % &\llama-\AD   & 37.2  & 19.8  & 43.6  & 51.9   && 26.1  & 9.2   & 27.9  & 43.3   \\
% % &\llama-\AQD  & 14.2  & 11.2  & 35.7  & 28.4   && 13.3  & 4.7   & 22.2  & 30.3   \\
% % &\llama-\AQDAnswer & 36.3  & 19.6  & 42.2  & 52.0   && 29.1  & 9.8   & 29.8  & 46.3   \\
% % &\llama-\QD   & 20.1  & 11.8  & 41.2  & 37.7   && 18.2  & 5.2   & 25.0  & 35.6   \\
% \cmidrule{2-11}
% &\multicolumn{10}{c}{\textbf{Oracle}}\\
% \cmidrule{2-11}

% &\gptF-\AQD   &  0.636 &  0.342  &  0.719  &  0.793   & & 0.556  & 0.156  &  0.437  &  0.799 \\
% &\gptF-\AQDAnswer  &  0.6   &  0.327  &  0.729  &  0.738   & & 0.56   & 0.156  &  0.435  &  0.818 \\
% &\gptF-\QD   &  0.66  &  0.337  &  0.678  &  0.837   & & 0.537  & 0.159  &  0.449  &  0.757 \\


% \midrule
% \midrule

% \multirow{3}{*}{\rotatebox{90}{\textbf{Learned Sparse (SPLADE)}}} & \\

% & \\
% & \\
% & \\
% & \\
% & \\
% & \\

% \cmidrule{2-11}
% &\multicolumn{10}{c}{\textbf{Oracle}}\\
% \cmidrule{2-11}

% & \\
% & \\
% & \\

% \bottomrule
% \end{tabular}

% }

% \end{table*}


% \gptF-\AQD   &  0.636 &  0.342  &  0.719  &  0.793   & & 0.556  & 0.156  &  0.437  &  0.799 \\
% \gptF-\AQDAnswer  &  0.6   &  0.327  &  0.729  &  0.738   & & 0.56   & 0.156  &  0.435  &  0.818 \\
% \gptF-\QD   &  0.66  &  0.337  &  0.678  &  0.837   & & 0.537  & 0.159  &  0.449  &  0.757 \\

% llama[G] & AQD  & 15.5  & 11.0  & 38.9  & 29.6   && 16.2  & 5.4   & 23.3  & 32.1   \\


\begin{table*}[t]
\centering
\caption{Passage retrieval results on TREC \cast 2020 and 2022 datasets. The best results that are significantly (t-test $p\_value \leq 0.05$) better are indicated by \textbf{$^{\ast}$} (Our comparison doesn't include the LLM4CS model). The best results are shown in \textbf{bold} and the second best results are shown with \underline{underline}. The best result outperforming all models is indicated by \textbf{$^{\ast}$}. The results for the LLM4CS model are reported from the original paper. In these experiments, we use the $\phi=5$.}
\vspace{-2mm}
\label{tab:retrieval-results-main-pool-cast}
\adjustbox{max width=1\textwidth}{
 \begin{tabular}{llllllllllll}
\toprule
\multirow{16}{*}{\rotatebox{90}{\textbf{Sparse (BM25)}}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c}{\textbf{\cast 2020}} & & \multicolumn{4}{c}{\textbf{\cast 2022}}\\ \cmidrule{3-6} \cmidrule{8-11}

&                     & \textbf{nDCG@3} & \textbf{R@100} & \textbf{MRR} & & \textbf{nDCG@3}  & \textbf{R@100} & \textbf{MRR}  \\
\cmidrule(lr){1-11} % similar way to create ctoprule(2-11)
&GPT4QR   & 46.8    & 55.2  & 61.5   && 34.8   & 30.1  & 52.2   \\
&T5QR     & 38.7   & 45.6  & 53.1   && 30.2   & 23.9  & 45.5   \\
&ConvGQR  & 35.7   & 47.7  & 49.4   && 25.0    & 22.1  & 41.0   \\
&LLaMAQR  & 33.3    & 44.0  & 46.0   && 22.1   & 21.8  & 39.3   \\
&LLM4CS   & 45.5     & 48.9  & 61.5   &&  -       &  -    &  -   \\
\cmidrule{2-11}
&HumanQR    & 50.5   & 61.8  & 66.8   && 41.3   & 37.6  & 60.4   \\
\cmidrule{2-11}
&\gptF-\AD   & 45.2   & 54.6  & 62.3   && 31.3  & 32.5  & 49.9   \\
&\gptF-\AQD  & 44.8   & 63.8  & 66.5   && 33.2    & 33.8  & 57.9   \\
&\gptF-\AQDAnswer & 45.0  & 57.6  & 62.9   && 32.5    & 35.0  & 51.6   \\
&\gptF-\QD   & 44.8  & 64.8  & 64.3   && 35.0    & 36.9  & 58.5   \\
% \cmidrule{2-11}
% &\llama-\AD   & 37.2   & 43.6  & 51.9   && 26.1  & 9.2   & 27.9  & 43.3   \\
% &\llama-\AQD  & 14.2    & 35.7  & 28.4   && 13.3  & 4.7   & 22.2  & 30.3   \\
% &\llama-\AQDAnswer & 36.3   & 42.2  & 52.0   && 29.1  & 9.8   & 29.8  & 46.3   \\
% &\llama-\QD   & 20.1   & 41.2  & 37.7   && 18.2  & 5.2   & 25.0  & 35.6   \\
\cmidrule{2-11}
&\multicolumn{10}{c}{\textbf{Oracle}}\\
\cmidrule{2-11}

&\gptF-\AQD   &  0.636   &  0.719  &  0.793   & & 0.556   &  0.437  &  0.799 \\
&\gptF-\AQDAnswer  &  0.6   &  0.729  &  0.738   & & 0.56     &  0.435  &  0.818 \\
&\gptF-\QD   &  0.66  &  0.678  &  0.837   & & 0.537   &  0.449  &  0.757 \\


% \midrule
% \midrule

% \multirow{3}{*}{\rotatebox{90}{\textbf{Learned Sparse (SPLADE)}}} & \\

% & \\
% & \\
% & \\
% & \\
% & \\
% & \\

% \cmidrule{2-11}
% &\multicolumn{10}{c}{\textbf{Oracle}}\\
% \cmidrule{2-11}

% & \\
% & \\
% & \\

\bottomrule
\end{tabular}

}

\end{table*}

==> tables/splade.tex <==


\begin{table}[h!]
\begin{tabular}{lcccccc}
\midrule
\midrule
cast20 & NDCG3 & NDCG & $r_{10}$ & $r_{100}$ & MRR@1000 \\
\midrule
QR Human &0.515& 0.645 &0.289 &0.684 &0.677\\
QR & 0.482& 0.613 &0.266& 0.631 &0.621\\
AD & 0.443 & 0.566 &0.230& 0.557& 0.624\\
\midrule
QD   & 0.432 & 0.612 &0.255 & 0.653 &   0.629 \\
AQD   & 0.423& 0.595 & 0.246 & 0.647  & 0.567 \\
AQDA & 0.458 & 0.585 & 0.249 & 0.578 & 0.629 \\
\midrule
cast20 oracle\\
\midrule
QD   & 0.609 & 0.687 &  0.333 & 0.749 & 0.760 \\
AQD   & 0.627& 0.683 & 0.342 & 0.730 &  0.805 \\
AQDA  & 0.658 & 0.668& 0.340 & 0.694  & 0.827 \\
\midrule
\\
\\
\\
\midrule
cast22 & NDCG3 & NDCG & $r_{10}$ & $r_{100}$ & MRR@1000 \\
\midrule
QR Human &0.432& 0.534 &0.140 &0.463 &0.619\\
QR &0.378 &0.487& 0.108 &0.394 &0.560 \\
AD &0.310 &0.427& 0.107 &0.354 &0.482\\
\midrule
QD   & 0.349 & 0.496 & 0.104 & 0.390 & 0.581 \\
AQD  & 0.332 & 0.477 & 0.093 & 0.359 & 0.571 \\
AQDA & 0.325 & 0.480 & 0.113 & 0.377 & 0.524 \\
\midrule
cast22 oracle \\
\midrule
QD   & 0.565 & 0.571 & 0.162 & 0.484 & 0.793 \\
AQD  & 0.565 & 0.573 & 0.172 & 0.481 & 0.796 \\
AQDA & 0.559 & 0.557 & 0.158 & 0.473 & 0.817 \\
\midrule
\\
\\
\\
\midrule
ikat23 & NDCG3 & NDCG & $r_{10}$ & $r_{100}$ & MRR@1000 \\
\midrule


QR Human &0.298& 0.356 &0.113 &0.295 &0.392\\

QR& 0.233 &0.303 &0.091 &0.284 &0.370\\
AD &0.159 &0.248 &0.074& 0.208 &0.256\\
\midrule
QD   & 0.225 & 0.318 & 0.075 & 0.305 & 0.409 \\
AQD  & 0.364 & 0.383 & 0.152 & 0.335 & 0.484 \\
AQDA & 0.101 & 0.238 & 0.045 & 0.173 & 0.181 \\
\midrule
ikat23 oracle \\
\midrule
QD   & 0.385 & 0.387 & 0.144 & 0.384 & 0.565 \\
AQD  & 0.476 & 0.436 & 0.201 & 0.437 & 0.642 \\
AQDA & 0.310 & 0.354 & 0.136 & 0.356 & 0.503 \\
\bottomrule
\end{tabular}
\centering
\caption{SPLADE GPT-4}
\label{tab:splade}
\end{table}


